Lachesis: Automatic Partitioning for UDF-Centric Analytics

Persistent partitioning is effective in avoiding expensive shuffling operations. However it remains a significant challenge to automate this process for Big Data analytics workloads that extensively use user defined functions (UDFs), where sub-computations are hard to be reused for partitionings compared to relational applications. In addition, functional dependency that is widely utilized for partitioning selection is often unavailable in the unstructured data that is ubiquitous in UDF-centric analytics. We propose the Lachesis system, which represents UDF-centric workloads as workflows of analyzable and reusable sub-computations. Lachesis further adopts a deep reinforcement learning model to infer which sub-computations should be used to partition the underlying data. This analysis is then applied to automatically optimize the storage of the data across applications to improve the performance and users' productivity.

==> README <==
This package provides a class for typesetting publications of the
Association for Computing Machinery.

Your TeX distribution probably includes the latest released version of
this package.  If you decide to install it yourself, please see the
Installation section of the User's Guide.

Please note that the version on Github is a development (or
experimental) version: please download it for testing new features.
The production version is the one on CTAN and ACM sites.


Changes

version 1.08    SIGPLAN reformatting (Matthew Fluet); bug fixes

version 1.09    SIGPLAN: revert caption rules (Matthew Fluet)

version 1.10    Bug fixes

version 1.11    Customization of ACM theorem styles and proof
                environment (Matthew Fluet).

version 1.12    Bug fixes and documentation updates.
                Footnotes rearranged.
                Option natbib is now mostly superfluous: the class
                makes a guess based on the format chosen.

version 1.13    Formatting changes: headers, folios etc.
                Bibliography changes.

version 1.14    Warn about undefined citation styles; move definitions
                of acmauthoryear and acmnumeric citation styles before
                use.

version 1.15    New structured affiliation command.
                New commands for acknowledgements.

version 1.16    Formatting changes for headers and footers.

version 1.17    Formatting changes for margins and lists.  Bug fixes.

version 1.18    Natbib is now the default for all versions.  A unified bib
                file is used for all styles.  Better treatment
                of multiple affiliations.

version 1.19    Include 'Abstract', 'Acknowledgements', and 'References'
                in PDF bookmarks.

version 1.20    Bug fixes, documentation updates

version 1.21    Bibliography changes: added arXiv, some cleanup

version 1.22    Bibliography changes for Aptara backend; should be
                invisible for the users.

version 1.23    Added PACM PL journal option.

version 1.24    Added IMWUT journal option.

version 1.25    Updated PACMPL journal option.

version 1.26    Bug fixes

version 1.27    Bug fixes

version 1.28    Bug fixes: natbib=false now behaves correctly.

version 1.29    Documentation changes.  Head height increased from 12pt to 13pt.
                Removed spurious indent at start of abstract.
                Improved kerning in CCS description list.

version 1.30    Bibtex style now recognizes https:// in doi.
                Added \frenchspacing.
                \department now has an optional hierarchy level.
                Switched to T1 encoding
                Updated IMWUT and PACMPL

version 1.31    Changed default year and month to the current ones
                (thanks to Matteo Riondato)
                Table of contents now works
                Marginalia now work in all formats
                New command \additionalaffiliation
                Documentation changes

version 1.32    New DOI formatting.
                Format siggraph is now obsolete, and sigconf
                is used instead.
                New proceedings title: POMACS.

version 1.33    New option `timestamp' (Michael D. Adams)
                New option `authordraft'
                Documentation updates
                Bug fixes
                We now use Type 1 versions of Libertine fonts even with XeTeX.
                New hook acmart-preload-hook.tex (wizards only!)
                Added new options `obeypunctuation' for \affiliation command
                Added SubmissionID
                Added right line count ruler for two-column formats
                Added workaround for Adobe Acrobat bugs in selection
                Added eid field to the bibliography

version 1.34    Deleted DOI from doi numbers
                Changed bibstrip formatting
                The command \terms is now obsolete
                The rulers in review mode now have continuous numbering

version 1.35    Author-year bib style now uses square brackets.
                Changed defaults for TOG sample
                Price is suppressed for usgov and rightsretained modes.
                Bugs fixed

Version 1.36    Bug fixes
                Moved PACMPL to acmlarge format
                New journal: PACMHCI
                Added the possibility to adjust number of author
                boxes per row in conference formats

Version 1.37    Reduce list indentation (Matthew Fluet)

Version 1.38    Increase default font size for SIGPLAN

Version 1.39    Added \authornotemark commmand

Version 1.40    Bibliography changes
                Added processing of one-compoment ccsdesc nodes
                Bug fixes.
                Made the height a multiple of \baselineskip + \topskip
                Added cleveref
                We no longer print street address in SIGs

Version 1.41    Rearranged bib files
                Added new badges

Version 1.42    Deleted ACM badges
                Bug fixes

Version 1.43    Bug fixes

Version 1.44    Bug fixes.
                Empty DOI and ISBN suppress printing DOI or ISBN lines
                Separated theorem code into acmthm.sty, loaded by default.
                Article number can be set for proceedings.
                New commands: \acmBooktile, \editor.
                Reference citation format updated.

Version 1.45    Workaround for a Libertine bug.  Thanks to LianTze Lim
                from Overleaf

Version 1.46    Bug fixes for bibliography: label width is now calculated
                correctly.
                All PACM now use screen option.  This requires etoolbox.
                Added subtitle to ACM reference format.
                Now acmart is compatible with fontspec.
                \thanks is now obsolete.  The addresses are automatically
                added to the journal version; this can be overriden with
                \authorsaddresses command.
                Deleted the rule at the end of frontmatter for all formats.
                Deleted new line before doi in the reference format.
                Reintegrated theorem code into acmart.dtx (Matthew Fluet)

Version 1.47    New journal: THRI

Version 1.48    Bug fixes
                Review mode now switches on folios
                Code prettying (Michael D. Adams)
                Bibliography changes: @MISC entries no longer have a
                separate date
                Sigch-a sample bibliography renamed
                Bib code cleanup (Zack Weinberg)
                Acmart and version info are added to pdfcreator tag
                \citeyear no longer produces parenthetical year
                Added initial support for Biblatex (Daniel Thomas)
                Added support for IW3C2 conferences

Version 1.49    New jorunal:  DTRAP

Version 1.50    Changes in iw3c2w3 and iw3c2w3g

Version 1.51    Journal footers now use abbreviated journal titles.
                Corrected the bug with acmPrice.
                Do not show price when copyright is set to iw3c2w3 and iw3c2w3g.
                The package now is compatible with polyglossia (Joachim Breitner).
                Slightly reworded copyright statements.

Version 1.52    Another rewording of licenses

Version 1.53    New journals: PACMCGIT, TIOT, TDSCI

Version 1.54    New option: 'nonacm' (Gabriel Scherer)
                Deleted indent for subsubsection (suggested by Ross Moore)
                Suppressed some obscurious warning in BibTeX processing
                Suppressed hyperrerf warnings (Paolo G. Giarrusso)
                New code for sections to help with accessibility patches
                (Ross Moore)
                Submission id, if present, is printed in anon mode
                Bug fixes

Version 1.55    Bug fixes
                Font changes for SIGCHI table captions

Version 1.56    Bug fixes
                Added \flushbottom to two column formats (Philip Quinn)
                The final punctuation for the list of concepts
                is now a period instead of a semicolon (Philip Quinn)
                New command \Description to describe images for visually
                impaired users.

Version 1.57    Change of \baselinestretch now produces an error
                Booktabs is now always loaded
                Added option `balance' to balance last page in two-column mode
                E-mail is no longer split in addresses
                New samples (Stephen Spencer)

Version 1.58    Suppressed spurious warnings.
		New journal:  HEALTH.
		TDSCI is renamed to TDS.

Version 1.59    Now a journal format can be used for conference proceedings
		All samples are now generated from the same .dtx file
		Bug fixes

version 1.60    New option: urlbreakonhyphens (thanks to Peter Kemp)
		Smaller header size for acmsmall

Version 1.61    Bug fixes
                New bibtex types for artifacts

Version 1.62    Documentation update
		New journal: TELO
		Bug fixes

Version 1.63	New journals: TQUANT, FACMP

Version 1.63a   Moved TQUANT to TQC

Version 1.64    Produce error if abstract is entered after maketitle
		(previously abstract was silently dropped)
		Bug fixes for line numbering

==> ir.tex <==
\section{\textit{Lachesis} IR}
In this section, we will describe our proposed IR.
\label{sec:ir}
For UDF expressions implemented in SparkSQL DSL~\cite{armbrust2015spark}, after an AST tree parsed from such an expression has been optimized, it is directly converted into Java byte code and the semantics are lost and a code snippet like \texttt{sup.startYear - 5} can not be extracted separately and re-invoked with new Supervisor objects in the future. Similarly, for an application represented in Weld IR~\cite{palkar2017weld} and Lara IR~\cite{kunft2019intermediate}, after these IRs have been optimized, the application is converted to LLVM IR, which is at assembly and register level, and the higher-level analyzable semantics, including the descriptions of sub computations are not persisted and all missing.

In addition, in order to partition a new dataset by reusing a sub computation from a UDF requires a number of functionalities: first, we need index each sub computation for extraction; second, to reuse and execute a sub computation for partitioning, we need  generate the code to customize a dispatcher, or create a partition computation and rewrite the IR to add it on the fly; third, to utilize the existing partitioning associated with a dataset when running a join operation, we need match the IR associated with the partitioning to the IR associated with the join computation to determine whether an expensive shuffling operation can be avoided. However, none of existing IRs provide these functionalities.

To address these problems, we propose a new IR, which is generated from the execution of our proposed DSL. 

\begin{figure}[H]
\centering{%
   \includegraphics[width=3.4in]{fig/fig2-graphIr.pdf}  
}%
\caption{\label{fig:graphIr}
Graph IR for the join$\langle$Department, Employee, Supervisor, SalaryGap$\rangle$
example: $O_i$ represents the $i$-th operator; and $L_j$ represents the
$j$-th lambda term following the lambda
term sequence number as shown in Fig.~\ref{fig:lambdaTree}.
}
\end{figure}



In our proposed graph
IR, each node represents an atomic computation that takes one or
more \texttt{vector}s of objects/references (which we call as a list
of \texttt{column}s) as input and outputs a new
list of \texttt{column}s.

Fig.~\ref{fig:graphIr} illustrates a non-optimized
Graph IR of a directed acyclic graph (DAG) of the following operators: three \texttt{scan} operators that
read objects from the ``deptSet'' \texttt{Set}, the ``empSet''
\texttt{Set}, the ``supSet'' \texttt{Set} respectively; a
\texttt{join} operator as described in Sec.~\ref{sec:join-example};
and a \texttt{write} operator that writes output to the ``myOut''
\texttt{Set}. The \texttt{join} operator takes the three \texttt{scan}
operators as input and outputs to the \texttt{write} operator.

In Fig.~\ref{fig:graphIr}, each node represents an atomic instruction (e.g. \texttt{\{$x_3$,startYear5\}=Minus(startYear,$l5$,$O_3$,$L_5$)}). 

Each instruction has three parts from left to right: 

\vspace{2pt}
\noindent
(1) \textbf{the list of output \texttt{column} names}, e.g. \{$x_3$, startYear5\} in above instruction,
with each \texttt{column} name representing a vector of objects output from the instruction. For example, in above instruction, $x_3$ represents a column of data elements that are kept from the output of the last instruction, i.e. \texttt{\{$x_3$, $startYear_1$, $l5$\}=Apply($O_3$, $L_5$)}, as shown in Fig.~\ref{fig:graphIr}. In addition, \texttt{startYear5} is a newly computed and appended column, which is generated from this instruction. Other column from the outputs of the last instruction, i.e. $l5$, is not shown in this part, so the column $l5$ should be removed and will not be output from this instruction. Each column has the same number of elements.

\vspace{2pt}
\noindent
(2) \textbf{the atomic computation
name}, such as \texttt{ScanSet}, \texttt{Apply}, \texttt{Hash},
\texttt{Filter}, \texttt{Flatten}, \texttt{Join}, \texttt{Aggregate}, \texttt{Partition},
\texttt{Equal}, \texttt{LessThan}, \texttt{Minus}, and \texttt{Multiply}. Each computation takes one or more columns as input, and outputs one or more columns. For example, in the above instruction, the \texttt{Minus} computation will substract the $k$-th element in the column $l5$ from the $k$-th element in the column $startYear_1$, and the substraction result will be added as the $k$-th element in the newly computed column \texttt{startYear5}.

\vspace{2pt}
\noindent
(3) \textbf{the
parameters taken by the atomic computation}, i.e. the input columns, the identifiers of the corresponding
lambda term and operator, from which code is generated through
C++ templates at compilation time. In the above instruction, the third part includes \texttt{(startYear, $l5$, $O_3$, $L_5$)}. \texttt{startYear} and \texttt{$l5$} are two input columns for the \texttt{Minus} computation; and \texttt{<$O_3$, $L_5$>} represents the indexing of this lambda term, which can be extracted and run independently.


Each atomic instruction can generate a new \texttt{column}, append it to the
output list, such as \texttt{ScanSet}, \texttt{Apply}, \texttt{Hash}, and
\texttt{Minus}; or combine several \texttt{column}s from different
lists into one list, such as \texttt{Join}. Each atomic instruction
also implicitly specify which \texttt{column}s should be kept as inputs for the next instruction,
which \texttt{column}s are not used anymore and should be removed from the
output list.

The IR can be persisted using PC object model~\cite{zou2018plinycompute}, and a lambda term indexed by $\langle O_i, L_j \rangle$ can be extracted to run from a historical IR to process new data.

\eat{
Based on lambda calculus DSL, the IR operates at a lower level than
Spark~\cite{zaharia2010spark}, 
and etc., so it can
expose more programming intentions for analysis and optimization.

Moreover, this IR operates at a higher
level than LLVM as used in Tupleware~\cite{crotty2015tupleware}, or
scala AST tree as used in the LMS~\cite{rompf2010lightweight}
framework. So the overhead for analysis and optimization is
significantly reduced compared to these systems. 
}

\subsection{IR Execution}
\label{sec:execution}
A lambda term can be a tree of lambda term abstractions and
lambda composing functions. A lambda composing function or a lambda term is also called as a
\texttt{Lambda} object, mapped to a node in the graph as illustrated in Fig.~\ref{fig:graphIr}. A \texttt{Lambda} object takes one or more inputs, which can be
the outputs from children \texttt{Lambda} objects.

Each \texttt{Apply} instruction is mapped to  a
\texttt{Lambda} object.
For example, in Fig.~\ref{fig:graphIr}, the instruction $\{x_1,
  name\}=$\texttt{Apply} $(x_1, O_3, L_0)$ means to execute the $0$-th lambda term
in Fig.~\ref{fig:lambdaTree}, which is \texttt{member($x_1$, name)},
while the executor code for applying this lambda term to a vector of
\texttt{Department} objects and obtain a vector of returned name strings, is generated by C++ templates at compilation
time. The code generation for other instructions is similar.

Each lambda composing instruction such as \texttt{Equal}, \texttt{Less-Than},
\texttt{Add}, and \texttt{Minus}, can be mapped to a higher
order function for composing lambda terms, such as \texttt{==}, \texttt{<},
\texttt{+}, \texttt{-}.

These instructions, as well as \texttt{Filter}, \texttt{Flatten}, and
\texttt{Hash}, are naturally data-parallel computations, which do not
need to materialize output data for broadcasting or shuffling. So a pipeline stage can be formed by a series of 
instructions like these, and can be easily executed using multiple threads
across many cluster nodes based on data parallelism.

In contrast, instructions such as \texttt{Join}, \texttt{Aggregate},
and \texttt{Partition}, often require to materialize output data
for broadcasting or shuffling. Such
instruction can be a pipeline breaker, which ends the processing of a pipeline,
materializes the pipeline output, broadcasts or shuffles the output across
the cluster, and then builds hash tables on the output if necessary so
that the hash tables can be probed
during the processing of next pipeline stages. 

The IR is designed that a physical optimizer can traverse it
and determine the join orderings and choose distributed join algorithms
dynamically based on runtime statistics such as the sizes of the
``deptSet'' \texttt{Set}, the ``empSet'' \texttt{Set}, and the ``supSet''
\texttt{Set}. Therefore, all instructions are implicitly parallel, and
programmers only need specify what to compute through the DSL and do not
need specify how to compute.


Most importantly, co-partitioning two data sets can avoid the resource-intensive shuffling process and speed up the distributed join and aggregation operations. In the following sections, we introduce how to enable co-partitioning of datasets automatically, which is a unique feature of our proposed IR.


\subsection{Lambda Term Extraction and Reuse}
Considering the example in Fig.~\ref{fig:graphIr}, if the ``empSet''
\texttt{Set} is partitioned based on the $x_2$->$getStartYear()$ method of each
\texttt{Employee} object $x_2$, and the ``supSet''
\texttt{Set} has been pre-partitioned based on the $x_3$->$startYear-5$ of each
\texttt{Supervisor} object $x_3$, the second \texttt{Join} instruction
that joins the ``empSet'' \texttt{Set} and the ``supSet''
\texttt{Set} has the opportunity to avoid shuffling or broadcasting
overhead and do a local
join on each partition. (In this case, if the ``deptSet'' \texttt{Set} has small
size and is chosen to be broadcast, the ``empSet''  \texttt{Set} will
not be re-partitioned for the first \texttt{Join}, and thus it will be
co-partitioned with the ``supSet'' \texttt{Set} for the second \texttt{Join}.)

We need identify which lambda term should be used to partition a dataset to be generated, which we will discuss in detail in Sec.~\ref{sec:optimization}. Here, we mainly discuss functionalities required from the IR: (i) Given a lambda term in a historical IR, how to identify, extract and reuse it in on-going applications; (ii) How to rewrite
the current IR that is being executed to partition a \texttt{Set} on the fly; (iii) When scheduling pipeline stages to run from an IR, how to match
the partition lambda term of the \texttt{Set} (i.e. $f_{partition}$ as
described in Sec.~\ref{sec:operations} ) to the join selection UDF
(i.e. $f_{sel}$ as described in
Sec.~\ref{sec:operations}), in order to determine whether it requires data shuffling and needs to break the pipeline or not. 

Such capabilities are unique
features of our graph IR, which are not only useful for
partitioning, but also useful for indexing and materialized view
creation. These capabilities do not exist in other object-oriented systems such as Spark~\cite{zaharia2010spark}, Flink~\cite{alexandrov2014stratosphere},
Weld~\cite{palkar2017weld}, Tupleware~\cite{crotty2015tupleware},
LMS~\cite{rompf2010lightweight}, and Lara~\cite{kunft2019intermediate}.

\subsubsection{Identify a Lambda Term}
While compiling DSL into IR, we store all lambda terms associated with
an operator into indexed trees, which is a variation of the Fenwick
tree~\cite{fenwick1994new}. All lambda terms are stored in an array
indexed by their sequence numbers in pre-order traversal, as shown as
the green labels in Fig.~\ref{fig:lambdaTree}. Each lambda term
stores:
\begin{itemize}
\item the root \texttt{Lambda} object which has a
\texttt{getExecutor()} member method for returning
generated code that applies the lambda function to a vector of
objects;
\item the indexes of its children lambda terms; \item the meta data of the
root \texttt{Lambda} object such as
the lambda function name (e.g. \texttt{member}), input type
(e.g. \texttt{Department}), parameters (e.g. attribute:\texttt{name}),
and output type (e.g. \texttt{String}).
\end{itemize}

Using such indexed tree structure, each
\texttt{Apply} instruction can efficiently locate a \texttt{Lambda} object in
$O(1)$ complexity. We can also use the index of the lambda term to
obtain the subtree rooted at a \texttt{Lambda} object to execute all instructions.

To extend the identification of lambda terms across different IRs, each
lambda term can be indexed by $<IR_i, O_j,
L_k>$, where $IR_i$ denotes the $i$-th IR, $O_i$ denotes the $j$-th operator, and $L_k$ denotes the
$k$-th lambda term associated with $O_j$. 

\subsubsection{Reuse a Lambda Term: Code generation and IR rewrite}
\label{sec:reuse}
To reuse a lambda term across applications, we need store the IR that
contains the lambda term to reuse. In the implementation, we store the compiled DSL in the form of
a DAG of compiled operator objects and a text
representation of the IR for ease of transmitting and development. The binary IR
structure can be easily derived from those.

There are generally two cases of reusing historical lambda term for
data partitioning: (1) to partition a dataset that is going to
be loaded from the client; (2) to partition a dataset that is going to be generated by
a computation at runtime.

We apply the \textbf{code generation} technique to the first case, which is to
utilize C++ templates to generate data dispatching code at the compilation
time, just like the generation of executor code. In result, the data
dispatcher first needs to locate the lambda term using $<IR_i, O_j,
L_k>$ in the historical IR, it then applies the root \texttt{Lambda}
object's \texttt{getDispatcher()} member
method, which returns the generated code, to run on each 
input object to extract the key for partitioning the object to one of
the workers.


For the second case, we apply the \textbf{IR rewrite} technique by 
creating and inserting a \texttt{partition} operator as described in
Sec.~\ref{sec:operations} to the current query graph. Because
\texttt{partition} operator is templated for input type and output
type, we can only create the object by invoking a
\texttt{createPartitionOp()} method from the
historical lambda term, which knows the input type (the input type of
leaf \texttt{Lambda} object nodes) and the output type (the output
type of the root \texttt{Lambda} object node).
The \texttt{partition} operator can specify $f_{keyProj}$ by the $<IR_i, O_j,
L_k>$ index, instead of using the historical lambda
calculus DSL that is lost in compilation. 

Then the DAG of operators and the
text
representation of IR are
updated to reflect the change and dispatched to workers at runtime for
running the job stage (i.e. a pipeline stage) to generate and partition the dataset. In
the same time, the historical IR that contains the lambda term
to be reused is also dispatched to workers. Then when each worker
thread executes the job stage, the lambda term will be
extracted from the historical IR and its executor will be invoked when
executing the on-going IR. 

The historical IR can be cached at worker nodes, so it only needs to
be transmitted once.


\subsubsection{Match a Lambda Term}
\label{sec:match}
When a physical optimizer is scheduling job stages to execute from IR, if it
meets an atomic instruction that is a potential pipeline breaker such
as \texttt{Join}, it needs to check whether both inputs for
\texttt{Join} are co-partitioned based on the lambda
term specified for the \texttt{Join} (e.g. as specified in $f_{sel}$ of the join operator), so that the optimizer can determine whether to avoid re-partitioning of input data.

To enable this, a \texttt{Set}'s partition lambda term, should be stored in form of the $<IR_i, O_j, L_k>$
index, a coarse-grained signature and a fine-grained signature. 

The coarse-grained signature is encoded based on the 
number of nodes in the lambda tree, height of the tree, and etc..

The fine-grained signature encodes the meta data information
(e.g. input type id, output type id, lambda function name id,
parameter strings) for each
\texttt{Lambda} object node in the tree in a deterministic order: using
breadth-first traversal and sorting sibling 
nodes that are children of any \texttt{Lambda} object representing commutative function, in lexicographical
order. 

Then the sequence of pipelined atomic computations: \texttt{Lambda} objects that run by
\texttt{Apply} instructions on the same input
\texttt{Set} and feed to a \texttt{Hash} instruction that is followed
by a \texttt{Join} instruction (i.e. hash partitioned join), or directly feeds to
a \texttt{Join} instruction (i.e. range partitioned join) and etc.,
will be used for matching. 

Firstly, the root \texttt{Lambda} object in the sequence will be located and its
index will be matched with the input \texttt{Set}'s partition lambda
term's index. If they match, the algorithm directly returns positive result. 

Otherwise, the coarse-grained signature for the \texttt{Lambda} object sequence used for \texttt{Join} will be generated to match with the input
\texttt{Set}'s coarse-grained signature. If they don't match, the
algorithm returns negative result.

In the end, the fine-grained signature for the \texttt{Lambda} object sequence
will be generated to match with the input \texttt{Set}'s fine-grained
signature. If they match, the algorithm returns positive result, otherwise it
returns negative result.







==> new-intro-punched.tex <==
\section {Introduction}
\label{sec:introduction}

%Predicted by IDC, by 2020 there will be $40$ zettabytes data on the earth, and $85$\% of the data are unstructured data that can not be represented in relational schemas~\cite{turner2014digital}. 
Big Data analytics systems such as Spark~\cite{zaharia2010spark}, Hadoop~\cite{white2012hadoop},  Flink~\cite{alexandrov2014stratosphere}, TupleWare~\cite{crotty2015tupleware}, and so on have been designed and developed to address analytics on unstructured data, which cannot be represented in relational schemas, and account for about 85\% of the data on earth~\cite{turner2014digital}. These systems use an API in high-level programming language such as Python, Java, or Scala. The APIs typically include operations such as \texttt{map()}, \texttt{reduce()}, \texttt{join()} and so on. Users can easily represent unstructured data as objects, and by supplying user-defined functions (UDFs) written in the host language to the operations, users can use control structures
such as conditional statements and loops to customize the computations.  Moreover, today's machine learning systems, such as TensorFlow~\cite{abaditensorflow}, PyTorch~\cite{paszke2017automatic}, scikit-learn~\cite{pedregosa2011scikit}, Ray~\cite{moritz2018ray}, and so on, are similar. In these systems, the training data and models are represented in tensors with arbitrary user-defined shapes, and the applications are implemented in python, which can be arbitrary compositions of lower-level operations for linear algebra computations, data manipulations, and so on, or even user-defined operations.

Such systems provide high flexibility and productivity and make it easy to develop complex analytics on top of unstructured data. However, a problem is that UDFs, operators, and workflows in these systems contain arbitrary codes that are opaque and deeply embedded in the programming language. It is not only hard to
reason about the logic of these arbitrary codes, but also hard to reuse sub-computations of opaque codes across libraries and applications for intelligent data pre-processing and pre-computation. Hence, standard physical database design such as automatic data placement that attempts to optimize the overall execution time for a set of applications is difficult. Specific challenges are:

\vspace{2pt}
1. \textit{How can an optimizer understand the semantics of a UDF such as a join condition embedded in the UDF?} Suppose there are two complex UDFs das following:

\begin{DSL}
vector<Item> getFrequentPurchased(Customer customer) 
{   //mine the most frequently purchased item set
    //from the all orders made by the customer.  }
vector<Item> getFrequentDiscounted(Supplier supplier) 
{   //mine the most frequently discounted item set
    //from all promotions posted by the supplier. }
\end{DSL}


\vspace{3pt}
Consider a join predicate expressed in a UDF as following:

\begin{DSL}
if (getFrequentPurchased(customer) ==
    getFrequentDiscounted(supplier)) return true;
else  return false;
\end{DSL}

The system  must understand that it is partitioning the set of Customer objects on the return value of method \texttt{getFrequentPurchased()}, and that it is partitioning the set of Supplier objects on the return value of method \texttt{getFrequentDiscounted}, in order to further understand whether it needs to shuffle either input dataset, or whether the data are already pre-partitioned appropriately across all cluster nodes.

\vspace{2pt}
2. One solution to the problem of opacity is to use a domain-specific language (DSL) that is understood by the system. But even in that case, in Big Data systems there is no information shared across computations; codes written in the DSL are compiled and then thrown away. \textit{How can the logic associated with the computation \texttt{getFrequentPurchased()} and \texttt{getFrequentDiscounted()} be extracted, stored, and indexed for reuse (e.g. pre-partitioning, creating indexing and materialized views, and so on) in future physical databse design and optimization?}

\vspace{2pt}
3. In a complex workload or workflow, a dataset might be used as input to multiple computations, which means there can be multiple candidate data organizations. In order to automatically choose an appropriate organization (such as a distributed partitioning scheme), \textit{how can the system accurately model the behavior of computations?}  Factors such as CPU cost, I/O cost and so on, are difficult to predict across different hardware configurations, different tuning parameters, and running over different data. 

\vspace{5 pt}
This problem of automatic physical optimization in a UDF-centric workload is related to but arguably more difficult than automatic, workload-based physical database design in relational databases~\cite{rao2002automating, agrawal2004integrating, nehme2011automated, zhou2012advanced, klonatos2014building}. SQL operates over highly structured relational data and the language is designed to expose programmer intent. It is well-understood how to compile an SQL query independent intermediate representation (IR)--relational algebra--from which it is easy to understand, extract and reuse various physical data organizations.

In this paper, we focus on automatically using historical workload information in a UDF-centric system to pre-compute and utilize physical data organizations for the underlying data. Our focus is specifically on computing and utilizing distributed pre-partitioning of the data to avoid shuffling. We know of no existing, UDF-centric system that is able to do this. 

A straightforward approach would be to analyze the IR provided by the host language such as Java or Scala (one could analyze the abstract syntax tree produced by the compiler). Some systems such as TupleWare~\cite{crotty2015tupleware} compile user application code into IR at AST level. However, this is unlikely to work in every case. It is difficult or impossible to reason about the behavior of user defined functions that encompass hundreds or thousands of lines of domain-specific code for operating over arbitrary objects. 

An alternative is to use a DSL rather than an opaque UDF to customize relational operators. The DSL can force the programmer to expose intent. This is the approach taken by SparkSQL~\cite{armbrust2015spark}, for example. Using the DSL, Spark can analyze the AST of the code and understand the semantics of an expression such as \texttt{employee1.startYear === employee2.endYear + 1}. 

However, after such an AST tree has been optimized, it is directly converted into Java byte code and the semantics are lost and a code snippet like \texttt{employee2.endYear + 1} can not be extracted separately and re-invoked in the future. This means that it cannot be used to perform workload-based optimization. Also SparkSQL DSL can not work with highly nested objects and arbitrary UDFs as to our knowledge.

Weld IR~\cite{palkar2017weld} and Lara IR~\cite{kunft2019intermediate} map python code to a high-level functional language. However, similar with SparkSQL DSL, the IR and the code generation are fully decoupled. This means if you want to reuse the code for some part of the IR, e.g. a function that maps an object to a key, you need first extract the IR fragment, modify it into a complete Weld IR program, and generate code from it using a compiler. This process is difficult to be automated. \eat{Particularly, Weld IR is not based on relational algebra and the join predicate is not structured, so it is difficult to identify and isolate the key extraction functions of join or aggregation operations for reusing these to pre-partition the datasets to be joined.} 

\vspace{5pt}
In this paper, we argue that object-oriented analytics systems should not only provide users a domain-specific language (DSL) to replace opaque UDF, but they should also compile programs written in the DSL into an IR that can be easily stored and reused to extract and apply user defined computations for automatic data placement. This IR should be higher-level than something like an AST, to permit fast, pattern-based processing without deep semantic analysis at a later time. While this IR should be based on relational algebra to facilitate extraction of join predicates, groupBy key extraction predicates, and so on, it should be lower level than relational algebra to capture the logic of UDF. Although we focus on reusing computation for data partitioning to avoid shuffling, the idea can also be applied to automated construction of materialized views, indexes and so on. 

We propose a DSL that includes a set of computations, which can be mapped to relational algebra operators like $select$, $join$, $aggregate$, and so on. Each of the computations contain structures such as selection function, projection function, key extraction function, and so on, which can be customized by user defined expressions. The DSL uses C++ templates to implement user defined expressions in the lambda calculus that link together atomic C++ codes.  For example, a join selection function \texttt{employee1.getStartYear() == employee2.endYear + 1} in our DSL is described as \texttt{method (employee1, getStartYear) == member (employee2, endYear) + 1}; and \texttt{getFrequentPurchased(customer) == getFrequentDiscounted(supplier)} is as \texttt{function (customer, getFrequentPurchased) == function( supplier, getFrequentDiscounted)}.

\texttt{method}, \texttt{member}, \texttt{function}, \texttt{==}, and \texttt{+} are all lambda composition functions that take as input lambda terms and return new higher-order lambda terms. These are all implemented as C++ templated functions for which efficient binary codes are generated at compilation time. At the same time, this codes are compiled into a unique IR, which can not only be analyzed by an optimizer, but also be stored for analysis and later reuse. For example, lambda terms like \texttt{member (employee2, endYear) + 1} can be easily indexed and in the future extracted and reused separately with new Employee objects. Similarly, \texttt{function (customer, getFrequentPurchased)} can be extracted as a standalone lambda term to generate partition keys for new Customer objects. This is a unique feature provided by our proposed IR. While our focus is on C++, our methods are for any language with appropriate macro facilities.

\vspace{5pt}
We further propose \textit{Lachesis}\footnote{\textit{Lachesis} is the name of a Greek God who allocates lots.}, which is an automatic data placement optimizer that is based on above lambda calculus IR. \textit{Lachesis} adopts a four-step, online approach to select and apply the optimal partition scheme for data to be loaded or generated into the system, or for intermediate data to be materialized by a computation. The steps are, whenever there is a data going to be loaded or generated:

\vspace{2pt}
\noindent
1. Recommend a candidate set of lambda terms based on historical workflow analysis, each of which specifies a workflow of atomic computations for deriving and appending the partition key for the data to be generated;

\vspace{2pt}
\noindent
2. Evaluate all candidates and select one using a cost-based approach and a deep reinforcement learning approach~\cite{sutton1998reinforcement};

\vspace{2pt}
\noindent
3. Apply the selected lambda term to partition data to be materialized via supplying a lambda term to the dispatcher, or via IR rewriting.

\vspace{2pt}
\noindent
4. Then, when a new operation is about to process the data, e.g. to perform a join or groupBy operation, the optimizer attempts to match the IR to recognize the lambda term that is used to partition the input data, and can decide whether such partition can be utilized for physical optimization, e.g. to perform a local join without re-partitioning data.

\vspace{5pt}
\noindent
\textbf{Our Contributions.}
To summarize, our contributions involve: (i) advocating a DSL based on the lambda calculus that is amenable to representation as a easily searchable, extractable and reusable IR; (ii)advocating to automatically analyze a database of such IRs and suggest reasonable physical organizations of data at runtime (when the data is to be generated); (iii)designing and comparing a cost-based and a deep reinforcement learning (DRL) approach for automatic data partitioning.

We demonstrate the benefits or our ideas by implementing it on top of \textit{PlinyCompute} ~\cite{zou2018plinycompute}, which is a high performance Big Data analytics computation framework developed in C++, and \textit{Pangea}~\cite{zou2019pangea}, which is a monolithic storage that closes the knowledge gap between computation and storage. 

The results show that Lachesis can achieve $2\times$ to $8\times$ performance speedup for TPC-H queries, linear algebra operations, and analytics applications with extremely low overhead. The results also show that the cost-based and the DRL-based approach can achieve similar results, while the DRL-based approach requires significantly longer time for training the model, and tuning hyper-parameters.









